Improving Transient Performance of Adaptive Control Architectures using Frequency-Limited System Error Dynamics

We develop an adaptive control architecture to achieve stabilization and command following of uncertain dynamical systems with improved transient performance. Our framework consists of a new reference system and an adaptive controller. The proposed reference system captures a desired closed-loop dynamical system behavior modified by a mismatch term representing the high-frequency content between the uncertain dynamical system and this reference system, i.e., the system error. In particular, this mismatch term allows to limit the frequency content of the system error dynamics, which is used to drive the adaptive controller. It is shown that this key feature of our framework yields fast adaptation with- out incurring high-frequency oscillations in the transient performance. We further show the effects of design parameters on the system performance, analyze closeness of the uncertain dynamical system to the unmodified (ideal) reference system, discuss robustness of the proposed approach with respect to time-varying uncertainties and disturbances, and make connections to gradient minimization and classical control theory.

==> Paper arXiv/macro.tex <==
\newfont{\smalll}{cmr8}
\def\ID{\hbox{I\hskip-.1em D}}
%\der\IR{\R}
% \def\IR{{\mbox{\hbox{I\hskip-.1em R}}}}
\def\IR{\mathbb{R}}
\def\IS{\mathbb{S}}
\def\zero{\mathbf{0}}
\def\one{\mathbf{1}}
\def\spec{\mathrm{spec}}
\def\diag{\mathrm{diag}}
\def\span{\mathrm{span}}
\def\eye{\mathrm{I}}
\def\Ir{{\mbox{{\smalll I\hskip-0.1em R}}}}
\def\IS{\hbox{I\hskip-.1em S}}
\def\IC{\hbox{C\hskip-
.5em\raise.5ex\hbox{$\scriptscriptstyle\mid$}}\ }
\def\Ic{\hbox{\smalll C\hskip-
.5em\raise.3ex\hbox{$\scriptscriptstyle\mid$}}\ }
\def\IE{\hbox{I\hskip-.1em E}}
\def\IN{\hbox{I\hskip-.1em N}}
\def\IP{\hbox{I\hskip-.1em P}}
\def\SS{\hbox{S\hskip-.4em S}}
\def\vtdef{ {\hskip 0.2em } _ {=} ^{\triangle } {\hskip 0.2em } }
\def\T={\buildrel {\scriptscriptstyle\triangle} \over =}
\newcommand{\ksum}[1]{\buildrel{\scriptscriptstyle #1}\over\oplus}
\def\open#1{\buildrel{\circ}\over{#1}}
\def\blkdiag{\mathop{\rm block{\scriptstyle -}diag}_
{i=1,2} }
\def\notin{\not\hskip-.0em\in}
\def\Empty{/\hskip-0.65em\odot} %\bigcirc}
\def\Empty{\mbox{\O}}
\def\cont{\mbox{\hskip -1 em\,}}
\def\CA{{\cal A}}
\def\CB{{\cal B}}
\def\CC{{\cal C}}
\def\CD{{\cal D}}
\def\CE{{\cal E}}
\def\CF{{\cal F}}
\def\CG{{\cal G}}
\def\CH{{\cal H}}
\def\CI{{\cal I}}
\def\CJ{{\cal J}}
\def\CK{{\cal K}}
\def\CL{{\cal L}}
\def\CM{{\cal M}}
\def\CN{{\cal N}}
\def\CO{{\cal O}}
\def\CP{{\cal P}}
\def\CQ{{\cal Q}}
\def\CR{{\cal R}}
\def\CS{{\cal S}}
\def\CSx{\CS_x}
\def\CT{{\cal T}}
\def\CU{{\cal U}}
\def\CV{{\cal V}}
\def\CW{{\cal W}}
\def\Cw{\small \CW}
\def\CX{{\cal X}}
\def\CY{{\cal Y}}
\def\CZ{{\cal Z}}
\def\CZx{\CZ_x}
\def\BA{\hbox{\bf A}}
\def\BB{\hbox{\bf B}}
\def\BC{\hbox{\bf C}}
\def\BD{\hbox{\bf D}}
\def\BE{\hbox{\bf E}}
\def\BF{\mbox{\bf F}}
\def\BG{\hbox{\bf G}}
\def\BH{\hbox{\bf H}}
\def\BI{\hbox{\bf I}}
\def\BJ{\hbox{\bf J}}
\def\BK{\hbox{\bf K}}
\def\BL{\hbox{\bf L}}
\def\BM{\hbox{\bf M}}
\def\BN{\hbox{\bf N}}
\def\BO{\hbox{\bf O}}
\def\BP{\hbox{\bf P}}
\def\BQ{\hbox{\bf Q}}
\def\BR{\hbox{\bf R}}
\def\BS{\hbox{\bf S}}
\def\BT{\hbox{\bf T}}
\def\BU{\hbox{\bf U}}
\def\BV{\hbox{\bf V}}
\def\BW{\hbox{\bf W}}
\def\BX{\hbox{\bf X}}
\def\BY{\hbox{\bf Y}}
\def\BZ{\hbox{\bf Z}}
\def\sqr#1#2{{\vcenter{\vbox{\hrule height.#2pt\hbox{\vrule
width.#2pt height#1pt \kern#1pt\vrule width.#2pt}\hrule
height.#2pt}}}}
\def\square{\mathchoice\sqr64\sqr64\sqr33\sqr33}
\def\diag{\mathop{\rm diag}}
\def\inf{\mathop{\rm inf}}
\def\block-diag{\mathop{\rm block{\scriptstyle -}diag}}
\def\limsup{\mathop{\rm lim\ sup}}
\def\liminf{\mathop{\rm lim\ inf}}
\def\pmbb#1{\setbox0=\hbox{#1}\raise 0.5ex\box0}
%\def\Cdot{\pmbb .}
\def\Cdot{\cdot}


\def\a{\alpha}
\def\b{\beta}
\def\e{\varepsilon}
\def\t{\theta}
\def\no{\noindent}
\def\s{\sigma}
\def\v{\vert}     \def\V{\Vert}
\def\ha{\hat A}
\def\l{\lambda}
\def\ckZ{\check Z}
\def\nxn{{n\times n}}
\def\underq{\underline q}
\def\underp{\underline p}
\def\underP{\underline P}
\def\RT{\hbox{\smalll T}}
\def\k{\kappa}
\def\L{\Lambda}
%\def\O{\Omega}
\def\o{\omega}
\def\s{\sigma}
\def\j{\jmath}
\def\g{\gamma}
\def\G{\Gamma}
\def\U{\Upsilon}
\def\D{\Delta}
\def\BD{{\bf \Delta}}
\def\d{\delta}
\def\norm#1{\|#1\|}
\def\onorm#1{|\!|\!|#1|\!|\!|}
\def\viks{\rm \vysmall {s}}
\def\vikm{\rm \vysmall {m}}

\def\tmin{\buildrel{\min}\over{\sim}}
\def\tablerule{\noalign{\hrule}}


\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{example}{Example}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{propo}{Proposition}[section]
\newtheorem{defintion}{Definition}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{problem}{Problem}[section]

\newcommand{\vtf}[4]{\left[ \begin{array}{c|c}
#1 & #2 \\ \hline #3 & #4 \end{array}\right]}

\newcommand{\mx}{_{\rm mixed}}
\newcommand{\fra}[2]{\mbox{$\frac{#1}{#2}$}}
\newcommand{\und}[1]{{\underline{#1}}}
\newcommand{\jmap}{:\j\IR\rightarrow\IC^{m\times m}}
\newcommand{\RC}{\IR\rightarrow\IC}
\newcommand{\RR}{\IR\rightarrow\IR}
\newcommand{\map}{:\IR\rightarrow\IR^{m\times m}}
\newcommand{\od}{\"{o}}
\newcommand{\Od}{\"{o}}

\newcommand{\etal}{{\it et al. }}
\newcommand{\bequ}{\begin{eqnarray}}
\newcommand{\eequ}{\end{eqnarray}}
\newcommand{\mT}{^\mathrm{T}}
\newcommand{\pr}{\mathrm{Proj}}
\newcommand{\rom}{\mathrm}
%\newcommand{\beqarray}{\begin{eqnarray}}
%\newcommand{\eeqarray}{\end{eqnarray}}
\newcommand{\Real}{{\mathbb{R}}}
\newcommand{\ra}{\rightarrow}
\newcommand{\nn}{\overline{\mathbb{R}}_+}
\newcommand {\subd}     {_{\rm d}}
\newcommand {\mathcalT} {{\mathcal{T}}}
\newcommand {\teq}      {\triangleq}
\newcommand {\mathcalG} {{\mathcal{G}}}
\newcommand {\sube}     {_{\rm e}}
\newcommand{\inv}{^{-1}}
\newcommand {\mathcalK} {{\mathcal{K}}}
\newcommand {\beq}      {\begin{equation}}
\newcommand {\eeq}      {\end{equation}}
\newcommand {\subu}     {_{\rm u}}
\newcommand {\mathcalD} {{\mathcal{D}}}
\newcommand {\subc}     {_{\rm c}}
\newcommand {\subF}     {_{\rm F}}
\newcommand {\mathcalX} {{\mathcal{X}}}
\newcommand{\Proj}{{\mathrm{Proj}}}
\newcommand{\tr}{{\mathrm{tr}}}
\newcommand {\submin} {_{\mathrm{min}}}
\newcommand {\submax} {_{\mathrm{max}}}
\newcommand{\col}{{\mathrm{col}}}
\newcommand {\mathrmC} {{\mathrm{C}}}
\newcommand{\BIS}{{\mathrm{BIS}}}
\newcommand {\subeff}    {_{\rm eff}}


%\newcommand{\T}{{\mathrm{T}}}


\def\Cone{{\rm C}^1}
\def\Hinf{{\rm H}_{\infty}}
\def\Htwo{\mbox{H}_2}
\def\Ltwo{{\rm L}_2}

\def\IR{{\mathbb R}}
\def\IC{{\mathbb C}}
\def\IE{{\mathbb E}}
\def\IN{{\mathbb N}}
\def\IP{{\mathbb P}}
\def\IS{{\mathbb S}}
\def\IT{{\mathbb T}}



\newcommand{\fb}{\hfill$\square$}
\newcommand{\inter}{\mathop{\cap}}
%\newcommand{\prod}{\mathop{\Pi}}
\newcommand{\union}{\mathop{\cup}}


\renewcommand\theenumi{\roman{enumi}}
\renewcommand\theenumii{\alph{enumii}}
\renewcommand\theenumiii{\arabic{enumiii}}
\renewcommand\theenumiv{\Alph{enumiv}}
\renewcommand\labelenumi{{\it\theenumi)}}
\renewcommand\labelenumii{(\theenumii)}
\renewcommand\labelenumiii{\theenumiii.}
\renewcommand\labelenumiv{\theenumiv.}

%Natasa's definitions

\def\Vs{V_{\rm s}}      %storage function               \Vs
\def\Va{V_{\rm a}}      %available storage              \Va
\def\rc{r_{\rm c}}      %supply rate - continious       \rc
\def\rd{r_{\rm d}}      %supply rate - discrete         \rd
\def\Wc{W_{\rm c}}      %supply rate - continious       \Wc
\def\Wd{W_{\rm d}}      %supply rate - discrete         \Wd

\def\CGc{\CG_{\rm c}}

\def\fc{{f_{\rm c}}}      %input - continuous             \fc
\def\fd{{f_{\rm d}}}      %input - discrete               \fd
\def\Gc{{G_{\rm c}}}      %input - continuous             \Gc
\def\Gd{{G_{\rm d}}}      %input - discrete               \Gd
\def\hc{{h_{\rm c}}}      %input - continuous             \hc
\def\hd{{h_{\rm d}}}      %input - discrete               \hd
\def\Jc{{J_{\rm c}}}      %input - continuous             \Jc
\def\Jd{{J_{\rm d}}}      %input - discrete               \Jd

%  for Controller
\def\fcc{f_{\rm cc}}      %input - continuous             \fcc
\def\fdc{f_{\rm dc}}      %input - discrete             \fdc
\def\Gcc{G_{\rm cc}}      %input - continuous             \Gcc
\def\Gdc{G_{\rm dc}}      %input - discrete               \Gdc
\def\hcc{h_{\rm cc}}      %input - continuous             \hcc
\def\hdc{h_{\rm dc}}      %input - discrete               \hdc
\def\Jcc{J_{\rm cc}}      %input - continuous             \Jcc
\def\Jdc{J_{\rm dc}}      %input - discrete               \Jdc


\def\Qc{Q_{\rm c}}      %input - discrete               \Qc
\def\Rc{R_{\rm c}}      %input - discrete               \Rc
\def\Sc{S_{\rm c}}      %input - discrete               \Sc

\def\Qd{Q_{\rm d}}      %input - discrete               \Qd
\def\Rd{R_{\rm d}}      %input - discrete               \Rd
\def\Sd{S_{\rm d}}      %input - discrete               \Sd

\def\Qcc{Q_{\rm cc}}      %input - discrete               \Qc
\def\Rcc{R_{\rm cc}}      %input - discrete               \Rc
\def\Scc{S_{\rm cc}}      %input - discrete               \Sc

\def\Qdc{Q_{\rm dc}}      %input - discrete               \Qd
\def\Rdc{R_{\rm dc}}      %input - discrete               \Rd
\def\Sdc{S_{\rm dc}}      %input - discrete               \Sd

\def\xc{x_{\rm c}}      %state - controller             \xc
\def\xe{x_{\rm e}}
\def\xci{x_{\rm c0}}
\def\uc{u_{\rm c}}      %input - continuous             \uc
\def\ud{u_{\rm d}}      %input - discrete               \ud
\def\yc{y_{\rm c}}      %output - continuous            \yc
\def\yd{y_{\rm d}}      %output - discrete              \yd

\def\ucc{u_{\rm cc}}    %input - continuous             \ucc
\def\udc{u_{\rm dc}}    %input - discrete               \udc
\def\ycc{y_{\rm cc}}    %output - continuous            \ycc
\def\ydc{y_{\rm dc}}    %output - discrete              \ydc
\def\rcc{r_{\rm cc}}    %supply rate - controller/cont. \rcc
\def\rdc{r_{\rm dc}}    %supply rate - controller/disc. \rdc

% DIMENSIONS
\def\mc{{m_{\rm c}}}      %                               \mc
\def\md{{m_{\rm d}}}      %                               \md
\def\lc{{l_{\rm c}}}      %                               \lc
\def\ld{{l_{\rm d}}}      %                               \ld
\def\pc{{p_{\rm c}}}      %                               \pc
\def\pd{{p_{\rm d}}}      %                               \pd

\def\mcc{m_{\rm cc}}      %                               \mc
\def\mdc{m_{\rm dc}}      %                               \md
\def\lcc{l_{\rm cc}}      %                               \lc
\def\ldc{l_{\rm dc}}      %                               \ld
\def\pcc{p_{\rm cc}}      %                               \pc
\def\pdc{p_{\rm dc}}      %                               \pd
\def\kapad{\kappa_{\rm d}}      %                               \pd
\def\kapac{\kappa_{\rm c}}      %                               \pd
\def\nc{n_{\rm c}}      %                               \nc

\def\Vr{V_{\rm r}}
\def\Vsc{V_{\rm sc}}

\def\CUc{\CU_{\rm c}}
\def\CUd{\CU_{\rm d}}
\def\Uc{U_{\rm c}}
\def\Ud{U_{\rm d}}

\def\CYc{\CY_{\rm c}}
\def\CYd{\CY_{\rm d}}
\def\Yc{Y_{\rm c}}
\def\Yd{Y_{\rm d}}

\def\CUcc{\CU_{\rm cc}}
\def\CUdc{\CU_{\rm dc}}

\def\CYcc{\CY_{\rm cc}}
\def\CYdc{\CY_{\rm dc}}
\def\sc{s_{\rm c}}

\def\CTc{\CT^{\rm c}}
\def\CTcc{\CT^{\rm c}_{\rm c}}
\def\CTcon{\CT_{\rm c}}

\def\CTcl{\tilde\CT}
\def\CTclc{\tilde\CT^{\rm c}}

\def\Ad{A_{\rm d}}
\def\Ac{A_{\rm c}}
\def\Bd{B_{\rm d}}
\def\Bc{B_{\rm c}}
\def\Cd{C_{\rm d}}
\def\Cc{C_{\rm c}}
\def\Dd{D_{\rm d}}
\def\Dc{D_{\rm c}}


\def\scq{s_{{\rm c}q}}
\def\fdq{f_{{\rm d}q}}
\def\fcq{f_{{\rm c}q}}
\def\IRc{{\overline{\IR}}}

\def\qc{q_{\rm c}}
\def\rc{r_{\rm c}}
\def\qd{q_{\rm d}}
\def\rd{r_{\rm d}}
\def\elc{\ell_{\rm c}}
\def\eld{\ell_{\rm d}}
\def\CWc{\CW_{\rm c}}
\def\CWd{\CW_{\rm d}}
\def\dc{d_{\rm c}}
\def\dd{d_{\rm d}}
\def\dcr{d_{\rm cr}}
\def\ddr{d_{\rm dr}}
\def\fcr{f_{\rm cr}}
\def\fdr{f_{\rm dr}}
\def\hcr{h_{\rm cr}}
\def\hdr{h_{\rm dr}}
\def\Gcr{G_{\rm cr}}
\def\Gdr{G_{\rm dr}}
\def\Jcr{J_{\rm cr}}
\def\Jdr{J_{\rm dr}}

\def\sc{s_{\rm c}}
\def\sd{s_{\rm d}}


%\newenvironment{proof}{{\bf Proof.}}{\hfill$\square$}

